Observations of planet forming disks in multiple stellar systems

The demographic of circumstellar disks, the birthplaces of planets, is diverse and rich in disks featuring rings, gaps, spirals, filaments, and arcs. Many studies revealing these disk structures have focused on objects around single stars and disks in isolation. The scenario is more complex if binarity or multiplicity is involved; most stars are part of multiple systems in crowded star-forming regions. How does the presence of one or more stellar companions affect the shape and size of the circumstellar disks? Here we review the landscape of results from optical, infrared, and (sub-) millimeter observations of the effects of multiplicity on protoplanetary disks, emphasizing the demographic studies of nearby molecular clouds and the high-resolution studies of multiple disk systems.

==> referee.tex <==
Major points:
- Section 2.3
A general comment about section 2 is that the authors are reporting disc dust sizes. We know that these radii are affected by radial drift. Radial drift differently affects single and multiple systems. I think it is important to stress this (there is a review by Francesco Zagaria that can be cited and citations therein). Specifically to Taurus, there is a study on disc sizes by Rota et al 2020 that compares gas radii. These could be more reliable in studying truncation. Also this work has to be cited.

A. We thank the referee for signaling the review and Rota et al. analysis. We added the references in the main text and changed Sec. 2 and 2.3 accordingly. 

- Section 3.2.2, par 1
The authors state that "spiral structures (are) expected from the gravitational collapse of a massive disc". This is wrong, discs need to be gravitationally unstable to form spirals, not necessarily to collapse. I also suggest citing a more general review on this topic. E.g. Kratter&Lodato 2016

A. We thank the referee for the suggestion. We corrected the main text and added the reference. 

- Section 4, par. 1
There is a debate about how mass from a circum-multiple disc distributes over the stars that is not reported in the review. There are studies (e.g. Dunhill+2015) that suggest deviations from the reported behaviour. In addition Ceppi et al 2022 studies this mechanism in systems with more than two stars, where also the possibility of mass equalisation is discussed. These additional comments have to be included for completeness.

A. We thank the referee for signaling us these papers. Dunhill+2015 found that if the companion is on a highly eccentric orbit, there is a strong precession of the disk and an even accretion on the two components, which may lead to keeping a mass ratio quite different from unity. We should then expect a correlation between eccentricity and mass ratio. This is now mentioned in the paper. Ceppi+2022 considered the case of triple hierarchical systems. They found that the smaller binary of a hierarchical triple accretes more mass than a single star of the same mass as the smaller binary. If the small binary is heavier than the third body, the standard differential accretion scenario (whereby the secondary accretes more of the mass) is hampered. Reciprocally, if the small binary is lighter than the third body, the standard differential accretion scenario is enhanced. We modified the text to include these points.

- Section 4, par 3
The systems added to Czekala et al. 2019 collection are:
- KH15D: The mutual inclination of this disc is reported as unknown in Czekala's paper. The articles cited are older than Czekala's paper. Is Czekala wrong and the mutual inclination is the one reported by the authors? Please check this.
- V773: Paper cited for the disc-orbit relative inclinations are all older than Czekala's paper. Is Czekala wrong in not reporting this additional disc? Kenworthy et al 2022 is more recent but, as far as I know, they do not observe the disc but just model a dimming in the stellar emission that could be associated with a highly inclined disc. I think this is not strong enough compared to the more strict selection Czekala et al made. This should be at least highlighted.
- T CrA: Can this misalignment be better justified?

A. Accurate determination of the mutual inclination requires knowledge of the Omega value for both disk and companion orbit. This is actually known only for a few cases - including that of T CrA whose paper is now published. In some additional cases, photometric modeling of occultation by a nearly edge-on disk may be used to constrain the inclination. This is the case for KH15D and V773 Tau. A recent model for KH15D has been proposed by Poon & Zhu (2021, MNRAS, 503, 1599) yielding a relative inclination in the range 5-16 degrees and r_in~1 au; these values are lower than those listed in Table 1. In the case of V773 Tau the relative disk-orbit inclination of 73 degrees that we considered is that indicated by the toy model used by Kenworthy et al. (2022). They give a small error bar, but the result might be a bit model dependent. We updated the paper accordingly.

- Section 4, par 5
Recently, Ceppi et al 2023 discuss the role of systems with more than two stars in the context of Figure 11 and Table 4. They showed that by considering multiplicity, the distribution in Figure 11 can be interpreted differently. Given what the authors said at the end of this paragraph, these additional insights into the distribution of mutual misalignment have to be reported.

A. We thank the referee for outlining this paper that was published after the first writing of our review and may indeed be relevant here. We now mention it in the text.

- Section 4, par 7,8
Chen+2020 discuss mainly the stability of planetary orbits. This is not the same as the stability of gaseous discs and this has to be highlighted. In addition, Chen+2020 concludes that polar orbits have a larger stable radial extend than coplanar ones. But, a polar disc behaves differently than a general not coplanar disc and extending this conclusion to all misaligned discs is not for granted. This has to be discussed.

A. The possibility to have stable polar gas disks at rather a short separation is discussed also in Doolin+2011, Martin+2018, and Cuello & Giuppone2019. We added citations of these papers and a sentence in agreement with the referee's point about the Chen+2020 paper.

- Section 4, par 9
When the authors compare the distribution of circumbinary planets by transit in Figure 12 they have to report that these detections are strongly biased towards coplanar orbits. This can weaken significantly the comparison done in Figure 12.

A. The argument here is that the frequency of multiple transiting systems is so high that requires that compact systems should have coplanar orbits. This is now spelled more clearly.

Minor points:
- Introduction, par. 4
Given the subsequent discussion about disc misalignment, I think it is important to report that also disc misalignment influences the truncation radius. See Lubow et al. 2015 and Miranda and Lai 2015

A. We added a phrase in the main text accordingly. 

- Section 2.1, par. 2
Is it possible to translate the flux ratio limits discussed in mass ratios? I think this information gives a better idea about the completeness of the survey

A. We added the value of the minimum observable mass since the mass ratio depends on the mass of the primary star, and in the case of Ophiuchus can be very wide. The flux-to-mass conversion has been calculated with evolutionary models. 

- Section 2.2
The authors report the age of Ophiuchus but not of Lupus (and Taurus later in the paper). Is it possible to add this information to better compare different surveys of stellar formation regions?

A. We added the values for the age of Lupus and Taurus in the text. 

- Section 2.2, par. 1
In the previous section, the authors state that in Ophiuchus all the identified discs are observed with ALMA. Is it possible to report this estimate also for Lupus? The idea is to quantify the "many" with which the second sentence of the section begins.

A. The phrase was probably confusing, the exact number (125) was stated just after. We removed the first part of the sentence and rephrased it to avoid confusion. 

- Section 2.2, par. 2:
The authors state that discs in multiples in Taurus are even smaller than in Ophiuchus. Are there information about the compactness of multiple systems in the two regions? Comparing the two regions, are generally smaller discs are associated with generally more compact systems?

A. The separations of the multiple systems for Lupus and Ophiuchus are shown in Figure 14 and Figure 9 of Zurlo et al. 2020 and 2021, respectively. Statistically, the two samples are not different. We modified the main text accordingly. removing the phrase "In the case of Lupus, the difference between multiple and isolated objects is even more dramatic than in Ophiuchus", and thank the referee to point that out. 

- Section 2.3:
Same comment as before about the age of Taurus

A. We added the value in the text. 

- Section 3.1, par. 2
It seems that Figure 8 is cited in the paper before Figures 6 and 7. Could this be fixed?

A. We have fixed the figures order. Additionally, we have restructured section 3 to improve the way the observations were presented. Basically, we moved the subsection "A word about formation pathways" to the beginning of section 3 as an introduction (now 3.1), and moved the paragraphs on SR24 to the end of section 3.1 (now 3.2). Only small edits to the text were made (marked in boldface) to improve readability. 

- Section 3.1, par 4
The authors say that in CHX 22 the arch-shaped feature is more likely produced by the interaction with the cloud rather than a flyby. A motivation or a citation to justify this statement is needed.

A. We added a citation to Dullemond et al. (2019) that presents cloudlet capture models which serve as motivation to compare with CHX 22. 

- Section 3.2.2, par 2
It is not completely clear what orientation the authors are discussing. Are the authors discussing the orientation relative to what? Between the orbital planes and disc planes? In this case, the conclusion of par. 2 is not the same as the conclusion of par. 3?

A. We thank the referee for pointing this out. We have edited the text to clarify and check for consistency between both paragraphs and decided to merge both paragraphs removing redundancies.  

- Section 3.2.2, par 7
Regarding the flyby nature of FU Ori outburst, the authors should cite Borchert et al 2022

A. We added the reference in the text. 

- Section 3.2.2, par 10
The authors say that HD98800 is "another" example of a polar aligned disc. Up to my knowledge, it is the only accretion disc we know is polar for sure. Which "other" examples are they referring to?

A. We replace "another prime example" with "a prime example". Although HD142527 is arguably a circumbinary disk with a binary with an almost polar inclination with respect to the outer disk, it is true that HD98800 is a clearer example.

- Section 4, par 5
When discussing Kozai-Lidov oscillations also Kozai should be cited (Kozai 1962)

A. We added the reference in the text. 

- Section 4, par 6
Same comment on V773 Tau and KH15D as in par 3

A. We corrected the inconsistency in the main text and updated the Figures. 

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


